Independent Subspace Analysis for Unsupervised Learning of Disentangled Representations

Recently there has been an increased interest in unsupervised learning of disentangled representations using the Variational Autoencoder (VAE) framework. Most of the existing work has focused largely on modifying the variational cost function to achieve this goal. We first show that these modifications, e.g. beta-VAE, simplify the tendency of variational inference to underfit causing pathological over-pruning and over-orthogonalization of learned components. Second we propose a complementary approach: to modify the probabilistic model with a structured latent prior. This prior allows to discover latent variable representations that are structured into a hierarchy of independent vector spaces. The proposed prior has three major advantages: First, in contrast to the standard VAE normal prior the proposed prior is not rotationally invariant. This resolves the problem of unidentifiability of the standard VAE normal prior. Second, we demonstrate that the proposed prior encourages a disentangled latent representation which facilitates learning of disentangled representations. Third, extensive quantitative experiments demonstrate that the prior significantly mitigates the trade-off between reconstruction loss and disentanglement over the state of the art.

==> lib.tex <==
% -*- compile-command: "texify --pdf --quiet PersonalizedHandTracking.tex" -*-
% Latex library functions
% Jamie Shotton
%
% With contributions from Chris Bishop and Antonio Criminisi

\usepackage{xspace}

	% JS notes
\definecolor{jscolornotes}{rgb}{0.2,0.6,0.2}
\definecolor{sicolor}{rgb}{0.1,0.1,0.6}
\newcommand{\js}[1]{\textcolor{jscolornotes}{[{\bf #1}]}}
\newcommand{\jsnote}[1]{\js{#1}} % LEGACY!
\newcommand{\jsremove}[1]{} % to remove JSnotes
\definecolor{xxawfcolor}{rgb}{0.6,0.2,0.2}
\newcommand{\xxawf}[1]{\textcolor{xxawfcolor}{\scriptsize[AWF: #1]}}
\newcommand{\SI}[1]{\textcolor{sicolor}{\scriptsize[SI: #1]}}
% ADD YOUR OWN COLOURS HERE!

\newcommand{\IGNORE}[1]{{}}

\newcommand{\defn}[1]{\textit{#1}}
\newcommand{\clslbl}[1]{#1}%\texttt{#1}}

\newcommand{\chapref}[1]{\chaptername~\ref{chap:#1}}
\newcommand{\Chapref}[1]{\chaptername~\ref{chap:#1}}
\newcommand{\chapsref}[2]{\chaptername s~\ref{chap:#1}~and~\ref{chap:#2}}
\newcommand{\Chapsref}[2]{\chaptername s~\ref{chap:#1}~and~\ref{chap:#2}}
\newcommand{\appref}[1]{\appendixname~\ref{chap:#1}}
\newcommand{\chaplabel}[1]{\label{chap:#1}}

%\newcommand{\secxref}[1]{Section~\ref{sec:#1}}
%\newcommand{\Secxref}[1]{Section~\ref{sec:#1}}
%\newcommand{\eqxref}[1]{(\ref{eq:#1})}
%\newcommand{\figxref}[1]{Figure~\ref{fig:#1}}
%\newcommand{\tablexref}[1]{Table~\ref{table:#1}}

% Generic reference commands
\newcommand{\seclabel}[1]{\label{sec:\reflabel-#1}}
\newcommand{\secref}[2][\reflabel]{\S\ref{sec:#1-#2}}
\newcommand{\Secref}[2][\reflabel]{\S\ref{sec:#1-#2}}
\newcommand{\secrefs}[3][\reflabel]{Sections~\ref{sec:#1-#2} and~\ref{sec:#1-#3}}

\newcommand{\eqlabel}[1]{\label{eq:\reflabel-#1}}
\renewcommand{\eqref}[2][\reflabel]{(\ref{eq:#1-#2})}
\newcommand{\Eqref}[2][\reflabel]{(\ref{eq:#1-#2})}
\newcommand{\eqrefs}[3][\reflabel]{(\ref{eq:#1-#2}) and~(\ref{eq:#1-#3})}

\newcommand{\figlabel}[2][\reflabel]{\label{fig:#1-#2}}
\newcommand{\figref}[2][\reflabel]{Fig.~\ref{fig:#1-#2}}
\newcommand{\Figref}[2][\reflabel]{Fig.~\ref{fig:#1-#2}}
\newcommand{\figsref}[3][\reflabel]{Figs.~\ref{fig:#1-#2} and~\ref{fig:#1-#3}}
\newcommand{\Figsref}[3][\reflabel]{Figs.~\ref{fig:#1-#2} and~\ref{fig:#1-#3}}

\newcommand{\alglabel}[2][\reflabel]{\label{alg:#1-#2}}
\newcommand{\algref}[2][\reflabel]{Algorithm~\ref{alg:#1-#2}}
\newcommand{\Algref}[2][\reflabel]{Algorithm~\ref{alg:#1-#2}}

\newcommand{\tablelabel}[2][\reflabel]{\label{table:#1-#2}}
\newcommand{\tableref}[2][\reflabel]{Table~\ref{table:#1-#2}}
\newcommand{\Tableref}[2][\reflabel]{Table~\ref{table:#1-#2}}

\newcommand{\jamie}[2][\reflabel]{#1-#2}

\newcommand{\reflabel}{dummy} % Dummy initial reflabel - use renewcommand...

\newcommand{\st}{\xspace\textrm{s.t.}\xspace}
\newcommand{\half} {\frac{1}{2}}
\newcommand{\intd} {\mathrm{d}}
\newcommand{\nth} {$^\textrm{th}$\xspace}

% Notes and to do
\newcommand{\note}[1]{{\color{blue} {\bf Note:} \it #1}}
\newcommand{\todo}[1]{{\color{red} {\bf To Do:} \it #1}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Chris Bishop
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\beas}{\begin{eqnarray*}}
\newcommand{\eeas}{\end{eqnarray*}}

\newcommand{\const}{{\rm const.}}
\newcommand{\matlab}{${\rm Matlab}^{\Pisymbol{psy}{226}}$}

% A comment
% XXX(sn) this macro is broken
%\newcommand{\comment}[1]{}

% Distributions
\newcommand{\normal}[2]{\mathcal{N}(#1 \given #2)}

%
\newcommand{\indep}{\bot \hspace{-0.6em} \bot}
\newcommand{\arrow}{\rightarrow}
\newcommand{\given}{\,|\,}
\newcommand{\twolines}{\,||\,}
\newcommand{\narroweq}{\!\!=\!\!}

% Parents and children
\newcommand{\pa}[1]{{\rm pa_\mathit{#1}}}
\newcommand{\cp}[2]{{\rm cp_\mathit{#1}^{(\mathit{#2})}}}
\newcommand{\ch}[1]{{\rm ch_\mathit{#1}}}

% Neighbours
\newcommand{\neigh}[1]{{\rm ne_\mathit{#1}}}

% KL divergence
\newcommand{\KL}{{\rm KL}}

% Entropy
\newcommand{\entropy}{{\mathbb{H}}}

% arg max
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}

%\providecommand{\ie}{}
%\providecommand{\eg}{}
%\providecommand{\etc}{}
%\providecommand{\etal}{}
%\providecommand{\vs}{}
%\providecommand{\cf}{}

%\newcommand{\ie}{i.e.~}
%\newcommand{\eg}{e.g.~}
%\newcommand{\etc}{etc.\xspace}
%\newcommand{\etal}{et al.\xspace}
%\newcommand{\vs}{vs.~}
%\newcommand{\cf}{cf.~}

\newcommand{\cip}{\mbox{$\perp\!\!\!\perp$}}
\newcommand{\condindep}[3]{#1~\cip~#2~|~#3}
\newcommand{\nocondindep}[3]{#1~\mbox{$\not\!\perp\!\!\!\perp$}~#2~|~#3}
\newcommand{\dir}[2]{{\rm Dir}(#1|#2)}

\newcommand{\bdelta}{\mbox{\boldmath $\delta$}}
\newcommand{\bDelta}{\mbox{\boldmath $\Delta$}}
\newcommand{\bbeta}{\mbox{\boldmath $\beta$}}
\newcommand{\bmu}{\mbox{\boldmath $\mu$}}
\newcommand{\bnu}{\mbox{\boldmath $\nu$}}
\newcommand{\balpha}{\mbox{\boldmath $\alpha$}}
\newcommand{\bepsilon}{\mbox{\boldmath $\epsilon$}}
\newcommand{\bgamma}{\mbox{\boldmath $\gamma$}}
\newcommand{\bSigma}{\mbox{\boldmath $\Sigma$}}
\newcommand{\btau}{\mbox{\boldmath $\tau$}}
\newcommand{\blambda}{\mbox{\boldmath $\lambda$}}
\newcommand{\bLambda}{\mbox{\boldmath $\Lambda$}}
\newcommand{\bpi}{\mbox{\boldmath $\pi$}}
\newcommand{\bpsi}{\mbox{\boldmath $\psi$}}
\newcommand{\bchi}{\mbox{\boldmath $\chi$}}
\newcommand{\bxi}{\mbox{\boldmath $\xi$}}
\newcommand{\bPsi}{\mbox{\boldmath $\Psi$}}
\newcommand{\bphi}{\mbox{\boldmath $\phi$}}
\newcommand{\bPhi}{\mbox{\boldmath $\Phi$}}
\newcommand{\btheta}{\mbox{\boldmath $\theta$}}
\newcommand{\bTheta}{\mbox{\boldmath $\Theta$}}
\newcommand{\bOmega}{\mbox{\boldmath $\Omega$}}
\newcommand{\bzeta}{\mbox{\boldmath $\zeta$}}

\newcommand{\Bmath}[1]{\mbox{\boldmath $#1$}}

\newcommand{\fastfig}[4]{
\begin{center}
\begin{figure}[htb!]
\centerline{\epsfig{figure=#1,width=#2}}
\caption[short]{#3}
\label{#4}
\end{figure}
\end{center}
}

\newcommand{\unit}{{\bf I}}
\newcommand{\boldzero}{{\bf 0}}

\newcommand{\bfa}{{\bf a}}
\newcommand{\bfb}{{\bf b}}
\newcommand{\bfc}{{\bf c}}
\newcommand{\bfd}{{\bf d}}
\newcommand{\bfe}{{\bf e}}
\newcommand{\bff}{{\bf f}}
\newcommand{\bfg}{{\bf g}}
\newcommand{\bfh}{{\bf h}}
\newcommand{\bfi}{{\bf i}}
\newcommand{\bfj}{{\bf j}}
\newcommand{\bfk}{{\bf k}}
\newcommand{\bfm}{{\bf m}}
\newcommand{\bfo}{{\bf o}}
\newcommand{\bfp}{{\bf p}}
\newcommand{\bfq}{{\bf q}}
\newcommand{\bfr}{{\bf r}}
\newcommand{\bfs}{{\bf s}}
\newcommand{\bft}{{\bf t}}
\newcommand{\bfu}{{\bf u}}
\newcommand{\bfv}{{\bf v}}
\newcommand{\bfw}{{\bf w}}
\newcommand{\bfx}{{\bf x}}
\newcommand{\bfy}{{\bf y}}
\newcommand{\bfz}{{\bf z}}

\newcommand{\bfA}{{\bf A}}
\newcommand{\bfB}{{\bf B}}
\newcommand{\bfC}{{\bf C}}
\newcommand{\bfD}{{\bf D}}
\newcommand{\bfE}{{\bf E}}
\newcommand{\bfF}{{\bf F}}
\newcommand{\bfG}{{\bf G}}
\newcommand{\bfH}{{\bf H}}
\newcommand{\bfI}{{\bf I}}
\newcommand{\bfK}{{\bf K}}
\newcommand{\bfL}{{\bf L}}
\newcommand{\bfM}{{\bf M}}
\newcommand{\bfO}{{\bf O}}
\newcommand{\bfP}{{\bf P}}
\newcommand{\bfQ}{{\bf Q}}
\newcommand{\bfR}{{\bf R}}
\newcommand{\bfS}{{\bf S}}
\newcommand{\bfT}{{\bf T}}
\newcommand{\bfU}{{\bf U}}
\newcommand{\bfV}{{\bf V}}
\newcommand{\bfW}{{\bf W}}
\newcommand{\bfX}{{\bf X}}
\newcommand{\bfY}{{\bf Y}}
\newcommand{\bfZ}{{\bf Z}}
\newcommand{\llangle}{{\langle \hspace{-0.7mm} \langle}}
\newcommand{\rrangle}{{\rangle \hspace{-0.7mm} \rangle}}
\newcommand{\define}{\stackrel{\mathrm{def}}{=}}

\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\La}{\left\langle}
\newcommand{\Ra}{\right\rangle}
\newcommand{\EXP}[1]{\left\langle #1 \right\rangle}
\newcommand{\vectwo}[2]{\left[\begin{array}{c} #1 \\ #2 \end{array}\right]}
\newcommand{\arrtwo}[2]{\begin{array}{c} #1 \\ #2 \end{array}}
\newcommand{\arrthree}[3]{\begin{array}{c} #1 \\ #2 \\ #3\end{array}}
\newcommand{\vecn}[1]{\left[\begin{array}{c} #1 \end{array}\right]}
%\newcommand{\half}{{\scriptstyle \frac{1}{2}}}
\newcommand{\col}{\mathrm{vec}}


\newcommand{\T}{{\rm T}}
\newcommand{\diag}{{\rm diag}}
\newcommand{\Tr}{\mbox{Tr}}
\newcommand{\diff}[1]{{\,d#1}}
\newcommand{\vgraph}[1]{
  \newpage
  \begin{center}
  {\large \bf #1}
  \end{center}
  \vspace{2mm}
}
\newcommand{\high}[1]{\textcolor{blue}{\emph{#1}}}
\newcommand{\cut}[1]{}
\newcommand{\citeasnoun}[1]{\citeN{#1}}
\newcommand{\citemulti}[2]{(#1, \citeyearNP{#2})}
\newcommand{\citemultiN}[2]{#1 (\citeyearNP{#2})}
\newcommand{\Sum}{{\displaystyle \sum}}

%%%
%%% Stuff for bold maths typesetting  ----------------------------------------
%%%
%%%   e.g. use "\bfmu" for boldface mu symbol
%%%
\def\bfmu{\mbox{\boldmath$\mu$}}
\def\bftau{\mbox{\boldmath$\tau$}}
\def\bftheta{\mbox{\boldmath$\theta$}}
\def\bfdelta{\mbox{\boldmath$\delta$}}
\def\bfphi{\mbox{\boldmath$\phi$}}
\def\bfpsi{\mbox{\boldmath$\psi$}}
\def\bfeta{\mbox{\boldmath$\eta$}}
\def\bfnabla{\mbox{\boldmath$\nabla$}}
\def\bfGamma{\mbox{\boldmath$\Gamma$}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% absolute value and norm
% http://tex.stackexchange.com/questions/43008/absolute-value-symbols

\usepackage{mathtools}

\DeclarePairedDelimiter\abs{\lvert}{\rvert}%
\DeclarePairedDelimiter\norm{\lVert}{\rVert}%

% Swap the definition of \abs* and \norm*, so that \abs
% and \norm resizes the size of the brackets, and the 
% starred version does not.
\makeatletter
\let\oldabs\abs
\def\abs{\@ifstar{\oldabs}{\oldabs*}}
%
\let\oldnorm\norm
\def\norm{\@ifstar{\oldnorm}{\oldnorm*}}
\makeatother

%%%

\DeclareMathOperator*{\rank}{rank}


